From Node Embedding To Community Embedding : A Hyperbolic Approach

Detecting communities on graphs has received significant interest in recent literature. Current state-of-the-art community embedding approach called \textit{ComE} tackles this problem by coupling graph embedding with community detection. Considering the success of hyperbolic representations of graph-structured data in last years, an ongoing challenge is to set up a hyperbolic approach for the community detection problem. The present paper meets this challenge by introducing a Riemannian equivalent of \textit{ComE}. Our proposed approach combines hyperbolic embeddings with Riemannian K-means or Riemannian mixture models to perform community detection. We illustrate the usefulness of this framework through several experiments on real-world social networks and comparisons with \textit{ComE} and recent hyperbolic-based classification approaches.

==> content/32-kmeans.tex <==
Given $n$ points $x_i \in \mathbb{B}^m$, Riemannian $K$-Means finds the barycenters $\mu_k$ of $K$ clusters and the label indicators $I_{nk}$ (equal to $1$ if $u_n$ is assigned to the cluster of barycenter $\mu_k$ and $0$ if not)  that minimises.
$$\sum_n \sum_k I_{nk}d^2(x_n,\mu_k)$$
Given some initialisation, $K$-Means perform the optimisation in two steps: the first updates each $I_{nk}$ to $1$ if $k = \arg \underset{j}{\min}\text{ }d^2(x_n, \mu_j )$ and $0$ if not, the second computes the barycenters given the updated indicators. For the latter step, we use Algorithm \ref{alg:barycenter} for numerical computation. To learn node clusters of GSD, we propose to apply $K$-Means on the embedding of in the Poincaré Ball. 


==> content/70-discussion.tex <==
\begin{itemize}
    \item Discuss how our approach improves the state of the art
    \item discuss comparisons with similar approaches
    \item discuss the choice of poincare ball model and why the graph data is hyperbolic in nature, why not use other manifolds 
    \item discuss the algorithmic choices
    \item discuss scalability of the approach
    \item  authors state that they have "to choose one embedding between several ones". A deep discussion should appear, with some references. As far as I know, hyperbolic embedding preserves the "intra-branch" distances of the hierarchy but not the positions of one branch regarding the others. Is this the kind of problem that the authors want to deal with? If so, would it be possible to redefine the loss to avoid the problem? If not, how many embeddings should be computed to be sure to have the "good" one?
    
    
    
\end{itemize}
